Coordinated Optical and Radar Measurements of Low Velocity Meteors

To better estimate which luminous efficiency ($\tau$) value is compatible with contemporary values of the ionization coefficient ($\beta$), we report a series of simultaneous optical and specular echo radar measurements of low speed meteors. A total of 1249 simultaneous EMCCD and radar meteors were identified. A subset of 36 events were analyzed in detail, with 29 having speed less than 20 km/s. These meteors had G-band magnitudes at the specular radar point between +4 and +7.7, with an average radiant power of 5W (assuming a 945 W power for a zero magnitude meteor) and masses of 1 - 10 mg. These correspond to a typical magnitude of +6. We find that $\beta$ / ${\tau}$ strongly correlates with radiant power. All our simultaneous meteors had asteroidal-like orbits and six were found to be probable iron meteoroids, representing 20 percent of our slow velocity sample. Luminous efficiency values averaged 0.6% at low speed, ranging from less than 0.1% to almost 30%. No trend of luminous efficiency with speed was apparent, though a weak correlation between higher values of luminous efficiency and radiant power may be present.

==> extras.tex <==
\subsection{Calibration plates}

Four distinct calibration plates are used operationally, and for data reduction. The \textit{calib} plate is the standard astrometric plate used for the wide-field camera, while the \textit{guide} plate is used for pointing the mirrors to any corresponding position on the wide-field image. The \textit{scale} and the \textit{exact} plate are used for obtaining high-precision measurements of meteor positions on narrow-field images. The description of each plate is given below, and a summary is given in Table \ref{tab:plates}.
    
\subsubsection{calib plate}
The \textit{calib} plate is a standard calibration plate which maps image pixel coordinate of the wide-field camera ($w_x$, $w_y$) to horizontal celestial coordinates ($\theta$, $\varphi$). The AST plate format is used for this purpose. The \textit{calib} plate can be made using METAL, whereby the user manually matches the stars on the image with the stars in the catalog until a satisfactory calibration is achieved, as described in \cite{weryk2012simultaneous}, section 3.3.


\subsubsection{guide plate}
When a meteor is detected on the wide-field system, the mirrors need to be steered to track it. For that purpose, the \textit{guide} plate is used. This plate maps image coordinates of the wide-field camera ($w_x$, $w_y$) to mirror encoder coordinates ($h_x$, $h_y$). As both coordinates are planar, the AFF plate format is used. This plate can be generated using the \textit{mosaic} program, which incrementally moves the mirrors across the sky and takes snapshots using the narrow-field camera to generate a mosaic image. The stars on this composite image are located and paired with the stars on the wide-field image to find the fit parameters. A more detailed description was given in \cite{weryk2013camo}, section 3.4. Another way of creating \textit{guide} plates is using the \textit{mircal} program, which uses data collected by \textit{mirchk}.


\subsubsection{scale plate}
For every video frame, the current mirror encoder position ($h_x$, $h_y$) corresponds to the centre of the narrow-field image ($n_x = 320$, $n_y = 240$). If one wants to convert the position of an object in the narrow-field image to celestial coordinates ($\theta$, $\varphi$), one first needs to find its position in mirror encoder coordinates (as outlined in the beginning of section \ref{section:data_calibration}), and use the \textit{exact} plate to convert them to ($\theta$, $\varphi$).

The \textit{scale} plate is used to convert the offsets from the centre of the narrow-field image ($\Delta n_x$, $\Delta n_y$) to the corresponding offsets in mirror encoder coordinates ($\Delta h_x$, $\Delta h_y$) and is implemented as an AFF plate. The plate should be stable against pointing changes, and it is only dependent on the optical setup and alignment. An initial version of the plate can be created with \textit{mosaic}, but a more accurate version can be created with \textit{mircal} and \textit{mirchk} (see section \ref{section: mirchk}).


\subsubsection{exact plate}

The \textit{exact} plate directly maps the mirror encoder coordinates ($h_x$, $h_y$) to the celestial horizontal coordinates ($\theta$, $\varphi$) and it is implemented as an AST plate. Paired with the \textit{scale} plate, this plate allows for high-precision trajectory estimation from measurements on narrow-field images. This plate is created using \textit{mircal} and \textit{mirchk}.

Before the \textit{exact} plate was introduced, narrow-field events were reduced by combining the \textit{guide} plate with the \textit{calib} plate, which was refered to as a ``boot-strapped'' fit. This effectively limited the measurement accuracy to the accuracy of astrometric calibration of the wide-field camera.

